Edge-Aware Curvature Modeling for Graph Understanding in Large Language Models

Recently, graph-aware Large Language Models (LLMs) have shown promising capabilities in jointly modeling graph-structured data and textual information. Existing approaches typically employ a graph encoder and a frozen LLM to obtain node representations from graph and textual views, followed by node-level alignment to bridge the two modalities. However, such alignment mechanisms primarily focus on node information while overlooking edge-level structures, leading to suboptimal information propagation across views. In this work, we conduct a comprehensive theoretical analysis to uncover why node-level alignment is insufficient for aligning textual and graph representations. Specifically, we prove theoretically for the first time that neglecting edge information leads to suboptimal solutions and negatively curved edges induce bottlenecked information flow, giving rise to the over-squashing phenomenon between graph and textual views. To address the two challenges, we innovatively proposed a CureLLM framework of Curvature-enhanced Graph Representations for Large Language Model whose goal is to inject the signals of edge information into the existing LLMs. Specifically, CureLLM first introduces the training-free textual prompt mechanism to make the LLM model generate the output directly based on the edge-aware prompt without learnable parameter costs. Furthermore, a novel curvature-aware graph representation learning is designed to capture the edge structure information to enhance the downstream tasks, where the message passing between text and graph representations only depends on edges with positive curvature. Finally, we conduct evaluations with 20 different compared methods on 11 real world datasets from various domains and the experiment results demonstrate the superiority of our proposed CureLLM framework.

==> Chapter/conclusion.tex <==

\section{Conclusion}


==> Chapter/experiments.tex <==
\iffalse
\begin{table}[]
\centering
\caption{Statistics of the datasets.}
\label{data_cf}
\renewcommand\arraystretch{1.5}
\resizebox{\textwidth}{!}{
\begin{tabular}{c||ccccc|cccc|cc}
\toprule
Dataset    & Instagram & Cora     & Citeseer & Photo      & WikiCS    & Baby       & Sports     & ML-1M     & ML-10M     & ExplaGraphs  & WebQSP        \\ \midrule
\# Nodes    & 11,339    & 2,708    & 3,186    & 48,362     & 11,701    & 26,495     & 53,955     & 9,746     & 80,555     & 2,766        & 4,737         \\
\# Edges    & 144,010   & 5,429    & 4,277    & 500,928    & 216,123   & 160,792    & 296,337    & 1,000,209 & 10,000,054 & 4.25(Avg)    & 4,252.37(Avg) \\
\# Features & 384       & 1,433    & 384      & 768        & 384       & 384        & 384        & 384       & 384        & 1,024        & 1,024         \\
Domain     & Social    & Academic & Academic & E-commerce & Wikipedia & E-commerce & E-commerce & Movie     & Movie      & Common Sense & Scene Graph  \\ \bottomrule
\end{tabular}}
\end{table}
\fi



\section{Experiments}
% Our experimentation focuses on the following research questions:
% RQ1: Can our framework enhance the performance in modeling TAGs compared with baselines? RQ2: Are all components comprising of the proposed method valid? RQ3: How do the hyperparameters impact the performance of the proposed method? RQ4: How do the different LLMs and GNNs impact the performance of the proposed method and how can optimal backbones be chosen? Due to the limitations of pages, the experiments about RQ3 and RQ4 are provided in \textbf{Appendix B}.
%In this section, we mainly presents a series of experiments and related analyses to validate the effectiveness of CureLLM. More details can be be referred to {\bf Appendix B}.
% In order to validate the effectiveness of CureLLM, we conduct extensive experiments on different datasets. Due to the limitations of pages, some experiments are provided in \textbf{Appendix B}.



\subsection{Experimental Setup}
\textbf{Datasets.} We evaluate the proposed method on three graph learning tasks: node classification \cite{graphadapter}, link prediction \cite{opengraph} and graph question answering (graphQA) \cite{G-retriever} using totally $11$ real-world datasets. These datasets have been widely adopted in previous literature \cite{engine}, \cite{wei2023multi}, \cite{bm3}, \cite{kong2024gofa}, \cite{G-retriever}. More information about the datasets and the relevant statistics are provided in {\bf Appendix B.1}.

\textbf{Implementation details.} For the classification task, following the existing settings \cite{tape}, we feed our learned fusion embeddings into a MLP head to obtain the final classification predictions. The widely-used \textit{Accuracy} metric is exploited to evaluate the classification performance. 
%
In link prediction task, we follow existing works \cite{wei2024multimodal}, \cite{opengraph} to conduct the full-rank test for each node, where the similarity of learned fusion embeddings can be calculated to predict the edge connection. To be specific, for each node, all nodes not connected to it in the training set are ranked by the model. The top-$K$ nodes are taken as positive predictions, and we calculate ${Recall@K}$ and ${Precision@K}$ scores with $K$ = $5$, $10$. 
%${Recall@K}$ is defined as the ratio of the number of true positive cases identified within the top $k$ results to the total number of positive cases. ${Precision@K}$ is the accuracy of evaluating the model in the top-$K$ prediction results.
%
For the GraphQA task, we follow the LLM head of existing work \cite{G-retriever}. Specifically,
the primary task of ExplaGraphs dataset is to assess whether
arguments are supportive or contradictory, using accuracy as the metric. For the WebQSP dataset, the $hit@1$ metric is used to assess the precision of the top returned answer. More implementation details are provided in {\bf Appendix B.2}.

\textbf{Baselines.} To verify the effectiveness of CureLLM, we compare it with traditional representaiton learning methods like MLP, MF, and the following representative and recent baselines, which can be mainly divided into three categories. \textbf{(1) GNN-based methods:} We select GCN \cite{gcn}, GAT \cite{GAT}, GIN \cite{GIN}, SAGE \cite{sage}, GraphCL \cite{GrapgCL}, CGCN \cite{CGCN}, and DSR-GNN \cite{DSR-GNN} as the compared methods.  \textbf{(2) Standard fine-tuned PLMs:} We select four widely used LMs: BERT(bert-base-uncased) \cite{bert}, DeBERTa (deberta-base) \cite{deberta}, SentenceBERT (bert-base-nli-mean-tokens) \cite{sentence-bert}, and RoBERTa (roberta-base) \cite{roberta}. \textbf{(3) LLM-enhanced methods:} We further compare the following state-of-the-art (SOTA) methods that combine LLMs and GNNs: WalkLM \cite{walklm}, TAPE \cite{tape}, OpenGraph \cite{opengraph}, ENGINE \cite{engine}, GraphAdapter \cite{graphadapter}, GraphToken \cite{graphtoken} and G-Retriever \cite{G-retriever}. Due to TAPE needs to obtain the interpretation of the text graph through GPT-3.5 and only the interpretation data on Cora is published. Therefore, we only report the classification results of this method on Cora. Besides, we also extend the baselines to our experiment setting of link prediction. Detailed descriptions for  the baselines can be found in {\bf Appendix B.3}.

%\textbf{Implementation details.} For the classification task, 

%We implement the proposed method using PyTorch. The example code of this work is provided in \textbf{supplementary material}. 
% Adam is adopted as the optimizer and the learning rate is searched in $\{1e-4, 5e-4\}$. In our experiments, we employ LLaMA2 \cite{llama2} as the default LLMs backbone and SAGE as an instance of GNNs. For LLMs, we specify a maximum tokenizer length of $512$ and a batch size of $8$ following the previous work \cite{hituner}. In the case of GNNs, our parameter configuration is follows: three layers, weight decay is set to $0$, and dropout rate is searched in $\{0.5, 0.6\}$. For a fair comparison, we run $5$ times and report the mean result and the standard deviation.
%Implementations of the baselines are either from open-source projects or the original authors. For the speciﬁc hyperparameters in the baselines, we use the values reported
%in their original literature. Additionally, we conduct our experiments on Nvidia GeForce RTX 3090 GPUs with 24GB memory. More experimental settings can be found in {\bf Appendix B.3}.

\begin{table}[t]
\centering
\caption{Accuracy(\%) of all compared methods on semi-supervised node classification task, where the best and runner-up performance are highlighted in bold and underlined respectively.}
\label{res_cf}
\renewcommand\arraystretch{1.5}
    \resizebox{0.85 \textwidth}{!}{
    \begin{tabular}{c||cccccc}
    \toprule
    Method       & Instagram             & Cora                  & Citeseer              & Photo                 & WikiCS                & \textit{Average}        \\ \midrule
    MLP          & 64.67 (0.31)          & 56.47 (0.97)          & 70.40 (1.08)          & 62.47 (0.25)          & 73.63 (0.35)          & 65.53          \\ \midrule
    GCN          & 64.54 (0.30)          & 79.53 (1.36)          & 69.78 (0.27)          & 83.01 (0.28)          & 79.51 (0.40)          & 75.27          \\
    SAGE         & 64.76 (0.45)          & 81.50 (0.69)          & 71.22 (0.24)          & 83.11 (0.29)          & 81.85 (0.29)          & 76.49          \\
    CGCN         & 65.67 (0.08)          & 81.50 (0.22)          & 69.60 (1.07)          & 64.74 (0.27)          & 80.95 (0.13)          & 72.49          \\
    DSR-GNN      & 64.52 (0.25)          & 76.77 (0.36)          & 71.11 (0.55)          & OOM                     & 78.91 (0.44)          & -              \\ \midrule
    BERT         & 62.42 (3.03)          & 62.36 (2.29)          & 67.02 (1.75)          & 73.57 (0.48)          & 81.18 (1.00)          & 69.31          \\
    DeBERTa      & 64.90 (1.52)          & 36.46 (9.55)          & 45.83 (17.2)          & 74.42 (0.38)          & 79.56 (2.90)          & 60.23          \\
    SentenceBERT & 62.75 (0.90)          & 62.07 (3.92)          & 67.08 (3.05)          & 73.38 (0.54)          & 80.61 (1.35)          & 69.18          \\ \midrule
    GraphAdapter & {\underline {67.45 (0.51)}}    & 78.03 (1.46)          & 70.50 (0.90)          & OOM                     & OOM                     & -              \\
    TAPE         & -                     & {\underline {84.91 (0.90)}}    & -                     & -                     & -                     & -              \\
    WalkLM       & 66.40 (0.29)          & 74.45 (3.19)          & 69.55 (1.17)          & 76.19 (0.21)          & {\underline {84.14 (0.61)}}    & 74.15          \\
    ENGINE       & 66.93 (0.51)          & 81.75 (1.06)          & {\underline {72.32 (0.81)}}    & {\underline {84.64 (0.14)}}    & 84.04 (0.47)          & {\underline {77.94}}    \\ \midrule
    Ours         & \textbf{68.30 (0.01)} & \textbf{85.31 (0.09)} & \textbf{73.92 (0.29)} & \textbf{86.31 (0.07)} & \textbf{84.80 (0.05)} & \textbf{79.73} \\ \bottomrule
    \end{tabular}
    }
\end{table}




% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\underlineine}{\underline}{}
\begin{table}[]
\centering
\caption{Performance(\%) comparison of baselines in terms of Recall@10, and Precision@10 on Baby, Sports, MovieLen-1M, and MovieLen-10M datasets. We mark the global best results on each dataset under each metric in boldface and the second best is underlined.}
\label{res_lp}
\renewcommand\arraystretch{1.5}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|cc|cc|cc|cc}
\toprule
Dataset      & \multicolumn{2}{c}{Baby}                    & \multicolumn{2}{c}{Sports}                  & \multicolumn{2}{c}{MovieLen-1M}              & \multicolumn{2}{c}{MovieLen-10M}            \\ \midrule
Model        & R@10                 & P@10                 & R@10                 & P@10                 & R@10                 & P@10                  & R@10                 & P@10                 \\ \midrule
MF           & 3.76 (0.22)          & 0.29 (0.04)          & 4.81 (0.29)           & 0.38 (0.0)            & 5.63 (0.28)           & 9.11 (0.42)            & 9.34 (0.53)          & 9.13 (0.31)          \\
MLP          & 3.94 (0.24)          & 0.31 (0.03)          & 4.96 (0.25)           & 0.40 (0.08)           & 5.88 (0.28)           & 9.23 (0.46)            & 9.52 (0.55)           & 9.36 
 (0.30)          \\ \midrule
GCN          & 4.17 (0.19)          & 0.34 (0.04)          & 5.08 (0.27)           & 0.41 (0.07)           & 6.02 (0.29)           & 9.32 (0.49)            & 9.96 (0.44)           & 9.55 
 (0.31)          \\
GAT          & 4.31 (0.19)          & 0.38 (0.04)          & 5.16 (0.22)           & 0.44 (0.08)           & 6.23 (0.29)           & 9.58 (0.49)            & 10.21 (0.52)          & 10.07 
 (0.32)         \\
GIN          & 4.21 (0.21)          & 0.36 (0.03)          & 5.09 (0.28)           & 0.43 (0.08)           & 6.14 (0.25)           & 9.43 (0.40)            & 10.24 (0.39)          & 9.89 
 (0.29)          \\
SAGE         & 4.67 (0.15)          & 0.42 (0.03)          & 5.46 (0.23)           & 0.49 (0.06)           & 6.47 (0.28)           & 9.86 (0.43)            & 11.33 (0.41)          & 10.57 (0.30)         \\
GraphCL      & 4.86 (0.16)          & 0.45 (0.03)          & 5.54 (0.20)           & 0.52 (0.05)           & 6.81 (0.22)           & 9.92 (0.36)            & 12.11 (0.44)          & 10.63 
 (0.28)         \\ \midrule
Bert         & 4.03 (0.21)          & 0.32 (0.05)          & 5.09 (0.22)           & 0.45 (0.07)           & 6.10 (0.24)           & 9.37 (0.38)            & 10.06 (0.51)          & 9.42 (0.30)           \\
RoBERTa      & 4.22 (0.18)          & 0.36 (0.03)          & 5.24 (0.20)           & 0.51 (0.07)           & 6.22 (0.28)           & 9.42 (0.48)            & 10.37 (0.48)          & 9.92 (0.28)           \\ \midrule
WalkLM       & 4.56 (0.12)          & 0.39 (0.02)          & 5.56 (0.23)           & 0.55 (0.04)           & 7.25 (0.21)           & 10.01 (0.35)           & 12.66 (0.42)          & 10.68 (0.24)          \\
GraphAdapter & 4.95 (0.15)          & 0.48 (0.02)          & 5.94 (0.19)           & 0.59 (0.04)           & {\underline{ 7.65 (0.24)}}     & {\underline {10.18 (0.38)}}     & {OOM}    & {OOM}    \\
OpenGraph    & 5.01 (0.11)          & 0.49 (0.03)          & 5.82 (0.22)           & 0.53 (0.05)           & 7.03 (0.21)           & 9.98 (0.34)            & 12.88 (0.39)          & 10.74 (0.23)          \\
TAPE         & {\underline {5.03 (0.12)}}    & {\underline {0.52 (0.02)}}    & {\underline {6.14 (0.19)}}     & {\underline{ 0.61 (0.04)}}     & 7.44 (0.23)           & 10.12 (0.35)           & \underline{13.68 (0.36)}          & \underline{10.81 (0.25)}          \\ \midrule
Ours         & \textbf{5.33 (0.11)} & \textbf{0.59 (0.01)} & \textbf{6.62 (0.16)} & \textbf{0.74 (0.04)} & \textbf{8.60 (0.19)} & \textbf{11.05 (0.32)} & \textbf{14.95 (0.33)} & \textbf{12.18 (0.20)} \\ \bottomrule
\end{tabular}}
\end{table}



\subsection{Overall Performance Comparison}
In order to evaluate the effectiveness of the proposed method, we compare the performance of our \methodbase framework to those of the baselines on different tasks.

\textbf{Node Classification.} We present the comparative analysis of node classification in Table \ref{res_cf}. 
% From the  experimental results, we derive the following observations: In general, \methodbase outperform all $12$ baselines on all datasets, showing the effectiveness of the proposed method in node classification task. The GNN-based methods outperform MLP on most datasets, indicating that structural information is crucial. Even though the performance of standard fine-tuned PLMs is not as good as that of GNN-based methods in general, they outperform MLP on some of the datasets, indicating that semantic information can not be ignored. 
% The ranking of many baselines is fluctuating across datasets, where the model of second-best performance scatters among GraphAdapter, TAPE, WalkLM, and ENGINE, showing the effectiveness of combining structural information and semantic information. Compared with the second-best performance, \methodbase achieves different levels of improvement on different datasets. In terms of average performance, the average performance of our framework is $1.79\%$ higher than the average performance of sub-optimal. This suggests that it is beneficial to consider edge attributes to align the graph and textual embeddings of the same node.
From the  experimental results, we derive the following observations: The ranking of many baselines is fluctuating across datasets, where the model of second-best performance scatters among GraphAdapter, TAPE, WalkLM, and ENGINE, showing the effectiveness of combining structural information and semantic information. Compared with the second-best performance, \methodbase achieves different levels of improvement on different datasets and average performance. This suggests that it is beneficial to consider edge attributes to align the graph and textual embeddings of the same node.



\textbf{Link Prediction.} We compare the link prediction results of our \methodbase to those of the baseline models. Table \ref{res_lp} shows the ${Recall@10}$ and ${Precision@10}$ on Baby, Sports, MovieLen-1M (ML-1M) and MovieLen-10M (ML-10M) datasets. In addition, we also conduct the experiments using the ${Recall@5}$ and ${Precision@5}$ metrics and the results are provided in {\bf Appendix B.4}.
% From Table \ref{res_lp}, we have the following observations: In general, \methodbase outperforms all $13$ baselines across all evaluation metrics on all datasets. It gains a substantial lead over the second-best models, TAPE and GraphAdapter, with performance improvements ranging from $6\%$ in ${Recall@10}$ on Baby to a significant $12.4\%$ on MovieLen-1M. Similar to the node classification task, baselines that combine structural and semantic information generally perform better than baselines that use one type of information alone. Compared LLM-enhanced methods, our \methodbase achieves the highest performance across all datasets, which also indicates the effectiveness of edge attributes.
From Table \ref{res_lp}, we observe that \methodbase outperforms all $13$ baselines across all evaluation metrics on all datasets, showing the effectiveness of the proposed method in link prediction task.

\textbf{Graph Question Answering.} Table \ref{res_qa} demonstrates the effectiveness of our method across the datasets. \methodbase obviously outperforms traditional prompt tuning and GraphToken, a graph prompt tuning-based method. Compared the state-of-art method G-Rtriever, \methodbase achieves $2.05\%$ higher than that on ExplaGraphs dataset and $2.09\%$ higher than that on WebQSP dataset. This suggests that utilizing edge attributes to align the graph and textual embeddings is also effective for graphQA task.

Overall, our \methodbase outperform all baselines across all evaluation metrics on all datasets in three tasks. This answers RQ1, showing that mining edge attributes for aligning the graph and textual information is capable of learning a more effective representation.

% 7.8 12.4 9
% \subsubsection{Node Classification}
% We present the comparative analysis of node classification in Table \ref{res_cf}. From the  experimental results, we derive the following observations:


% \subsubsection{Link Prediction}
% \subsubsection{Graph Question Answering}

\begin{table}[htbp]
    \centering
    \begin{minipage}{0.38\textwidth}
        \centering
        \large
        \caption{Performance comparison across ExplaGraphs and WebQSP.}
        \label{res_qa}
        \resizebox{\linewidth}{!}{
        \begin{tabular}{ccc}
            \toprule
            Method & ExplaGraphs & WebQSP \\ \midrule
            Prompt tuning & 57.63 (2.43) & 48.34 (0.64) \\
            GraphToken & 85.08 (5.51) & 57.05 (0.74) \\
            G-Retriever & \underline{85.16 (0.92)} & \underline{70.49 (1.21)} \\ \midrule
            Ours & \textbf{87.21 (0.85)} & \textbf{72.58 (0.51)} \\ \bottomrule
        \end{tabular}}
    \end{minipage}
    \hspace{0.01\textwidth} % 增加间距
    \begin{minipage}{0.59\textwidth}  % 减小宽度
        \centering
        \caption{Ablation study of CureLLM where w/o denotes the removal of a specific component.}
        \label{ablation_cf}
        \resizebox{\linewidth}{!}{ % 自动缩放表格
        \begin{tabular}{l|ccccc} \toprule
               & Instagram & Cora & Citeseer & Photo & WikiCS \\ \midrule
            \textit{w/o} structural information & 64.51 & 72.88 & 69.28 & 73.25 & 81.46 \\
            \textit{w/o} semantic information & 64.76 & 81.50 & \underline{71.22} & 83.11 & 81.85 \\
            \textit{w/o} inference ability & \underline{67.33} & 73.25 & 61.91 & 84.92 & 81.25 \\
            \textit{w/o} edge attribute & 66.84 & \underline{83.03} & 70.85 & \underline{85.67} & \underline{83.34} \\ \midrule
            CureLLM & \textbf{68.30} & \textbf{85.31} & \textbf{73.92} & \textbf{86.31} & \textbf{84.80} \\ \bottomrule
        \end{tabular}}
    \end{minipage}
    
\end{table}












\subsection{Ablation Study}
We evaluate all components by removing each item from \methodbase in turn: (a) \textit{w/o} structural information: replacing GNN with MLP; (b) \textit{w/o} semantic information: removing textual embedding; (c) \textit{w/o} inference ability: replacing Llama2 with DeBERTa; (d) \textit{w/o} edge attribute: removing curvature-based alignment. The experiment results of node classification are presented in Table \ref{ablation_cf} and more experiment results can be found in {\bf Appendix B.5}. From Table \ref{ablation_cf}, we can observe that removing any components may lead to a decrease in performance.
%Overall, removing structural information in the most significant performance drop across all datasets, aligning with the nature of text-attribute-graphs that structure-related information plays a more pivotal role than pure text. Disabling inference ability reveals that such knowledge significantly enhances performance, indicating the generalizable knowledge derived from LLMs remains valuable. The result of removing the edge attribute reveal that the message passing between text and graph representations only depends on edges with positive curvature benefits the final representation learning.

\subsection{Case Study}
In order to investigate the effect of different hyperparameters and the effect of different components of LLMs and GNNs, we also conduct hyperparameter experiments and the comparison with different LLM-based models, which are provided in \textbf{Appendix B.6} and \textbf{Appendix B.7}.


\vspace{-1mm}
\section{Conclusion}

 In this work, we alleviate the problem of partial alignment in the existing graph-aware large language model from the perspective of curvature for the first time. Based on the theoretical analysis, we proposed a novel \methodbase framework whose goal is to exploit the signals of edge attributes to enhance the existing alignment mechanism.
 %Our proposed \methodbase comprehensively analyzes the shortcomings of existing textual-graph alignment mechanisms, where we prove theoretically the limitations: (1) the lack of edge information
%can lead to a suboptimal solution and (2) the edges with negative curvature are the main reason for the information bottleneck. Based on the theoretical analysis, we proposed a novel \methodbase framework whose goal is to exploit the signals of edge attributes to enhance the existing alignment mechanism. Extensive experiments show the superiority of our proposed method in terms of test performance for the graph downstream tasks.




% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\underlineine}{\underline}{}




% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \begin{table}[]
% 	\centering
%         \caption{}
% 	\label{res_qa}
% 	\begin{tabular}{ccc}
% 		\toprule
% 		Method        & ExplaGraphs  & WebQSP       \\ \midrule
% 		Prompt tuning & 57.63 (2.43) & 48.34 (0.64) \\
% 		GraphToken    & 85.08 (5.51) & 57.05 (0.74) \\
% 		G-Retriever   & 85.16 (0.92) & 70.49 (1.21) \\ \midrule
% 		Ours          & 87.21 (0.85) & 72.58 (0.51) \\ \bottomrule
% 	\end{tabular}
% \end{table}


% \begin{table}[]
% \centering
% \caption{Ablation study of CureLLM where w/o denotes the removal of a specific component.}
% \label{ablation_cf}
% % \resizebox{\textwidth}{!}{
% \begin{tabular}{l|ccccc} \toprule
%        & Instagram      & Cora           & Citeseer       & Photo          & WikiCS         \\ \midrule
% \textit{w/o} structural information & 64.51          & 72.88          & 69.28          & 73.25          & 81.46          \\
% \textit{w/o} semantic information   & 64.76          & 81.5           & \underline{71.22}          & 83.11          & 81.85          \\
% \textit{w/o} inference ability      & \underline{67.33}          & 73.25          & 61.91          & 84.92          & 81.25          \\
% \textit{w/o} edge attribute         & 66.84          & \underline{83.03}          & 70.85          & \underline{85.67}          & \underline{83.34}          \\ \midrule
% CureLLM                       & \textbf{68.30} & \textbf{85.31} & \textbf{73.92} & \textbf{86.31} & \textbf{84.80} \\ \bottomrule
% \end{tabular}
% \end{table}



\clearpage


==> Chapter/introduction.tex <==



\section{Introduction}
\noindent{\bf (Background.)} With the rapid growth of online data scale \cite{luo2024chatkbqa, DBLP:conf/nips/DuLJLN24}, the large language models (LLMs) have achieved great success in many domains \cite{ren2024survey, hu2024uncertainty, NEURIPS2024_305b2288}. 
%
In order to transfer the rich knowledge of LLMs to the practical tasks based on the graph-structured data \cite{lin2023automatic}, such as recommender systems \cite{lin2024enhancing}, social networks \cite{DBLP:conf/kdd/MengWHL0Z24} and disease prediction \cite{DBLP:conf/www/0002TZ025},  graph-aware LLMs have become a critical research area in recent years \cite{DBLP:conf/nips/0001WZCJ0C024, wang2023can}.
%
To enable LLMs to recognize graph structure data, most previous research \cite{tang2024higpt} has explored
projecting the
textual attributes and graph topology structure into the same latent space to enhance the 
 representation learning in LLMs. Specifically, as illustrated in Fig. \ref{toy2}(a), the existing graph-textual paradigm of LLMs may use the frozen LLM encoder and trainable graph adapter to extract the textual and graph embeddings for the node $v_1$. Then, some alignment mechanism, such as supervised learning \cite{chen2023agnn} or contrastive learning \cite{wei2024llmrec}, is adopted to align the node embeddings under textual and graph views for node $v_1$. 


\noindent{\bf (Limitations.)} 
%
However, the above graph-textual alignment mechanism only serves the node embeddings as the bridge to align textual and graph views while ignoring the edge attributes of the graph, which may hinder the graph understanding of LLMs.
%
Taking Fig \ref{toy2}(b) as an example, we conduct an experimental analysis of the existing graph-aware LLMs \cite{DBLP:conf/sigir/Tang00SSCY024} and visualize the representation distribution with the proposed node-aligned mechanism. From the results, we can observe that only using node information can lead to partial alignment, especially the nodes located at the decision boundary can not be well distinguished.


\begin{figure}[t]
    \centering
    \label{toy2}
\includegraphics[width=1\linewidth]{Fig/toy2.pdf}
    \caption{A toy example of large language models (LLMs) with graph understanding.
    (a) The existing paradigm of graph-textual LLMs;
    (b) The limitations of existing graph-textual alignment mechanisms in LLMs;
    (c) The illustration for graph curvature.
    }
\end{figure}




\noindent{\bf (Motivations.)} 
%
%Ignoring the attribute information of the edges may be one of the reasons for the above problems. 
%
To explain the above phenomenon, we first attempt to analyze the existing paradigm of graph-aware LLMs from a theoretical perspective. Then, we surprisingly find that the sub-optimal solution for the above aligned representations can be attributed to the lack of edge information (see {\bf Theorem 1} in Section \ref{motivation_theorem}). 
%
Based on discovery of {\bf Theorem 1}, we continue to study the properties of edge attributes in the graph-aware LLMs, where we further find that the edges with negative curvature are the main reason for the information bottleneck between graph and textual views (see {\bf Theorem 2} in Section \ref{motivation_theorem}). 
%
Here, we hope to use a simple toy example to help understand our theoretical findings, as shown in Fig. \ref{toy2}(c).
%
{\bf Theorem 1} points out the drawback of the existing textual-graph alignment mechanism in LLMs. For example,
if the message between textual and graph views is aligned only through a common node (e.g., the  node $v_1$ under the textual view  $\rightarrow$ the node $v_1$ under the graph view), the information between different views can be squeezed into a fixed-size feature space (e.g., the dark green dotted line from nodes $v_1, v_2, v_3, v_4$ and $v_5$ under the graph view to nodes $v_1$ under the textual view). 
%
The above problem with squashing of exponentially growing amount of information into fixed-size node features, which hinders the message passing between
nodes, is termed as "over-squashing" phenomenon in the previous works \cite{DBLP:conf/icml/AttaliBP24, attali2024delaunay}. {\bf Theorem 2} aims at introducing curvature to analyze the above problems. Curvatures of edges are the tools from differential geometry \cite{chami2019hyperbolic} to measure how difficult it is for the information to propagate between two nodes \cite{ye2019curvature}, where negative curvature means it is hard for information to pass. Through the tools of curvature \cite{fu2025discrete}, we can model the information transfer between textual and graph views in LLMs as a geometric manifold, as shown in the right part of Fig. \ref{toy2}(c). Then, we are surprised to find that the over-squashing problem in LLMs can correspond to the information bottleneck caused by the negative curvature ($\boldsymbol{\kappa} \textless 0$) in the geometric manifold (Ricci flow).

\noindent{\bf (Solutions.)} 
Inspired by the above theoretical motivations, we hope to exploit the edges with positive curvatures to enhance the existing textual-graph alignment mechanism in LLMs. Therefore, we innovatively proposed a \methodbase framework of {\bf Cur}vature-{\bf e}nhanced Graph Representations for {\bf L}arge {\bf L}anguage {\bf M}odel, consisting of the training-free textual prompt mechanism and curvature-aware graph representation learning, where our \methodbase considers aligning the textual and graph representations based on the positive curvature while filtering the negative curvature. For the training-free textual prompt mechanism, a novel prompt mechanism for pre-trained models is designed to predict the desired output without any additional task-specific training, which can reduce the cost of training. For the curvature-aware graph representation learning, a two-step curvature alignment enhancement is exploited to alleviate the information bottleneck between the graph and textual views. Then, after the alignment mechanism, the obtained final textual-graph
fusion representations are fed to the different heads for various downstream tasks.

\noindent{\bf (Contributions.)}
The contributions of this paper are outlined as follows. \emph{ (1) About Novelty:} To the
best of our knowledge, our work is the first to introduce the curvature into the LLMs, which establishes the connection between LLMs
and Riemannian geometry for the first time.
\emph{(2) About Effective Model Design:} Our \methodbase is the first framework to exploit the edge attributes to enhance the alignment between textual and graph representations in graph-aware LLMs. \emph{(3) About Theoretical Analysis:}  We prove theoretically for the first time that the lack of edge information
can lead to a suboptimal solution, and the edges with negative curvature are the main reason for the information bottleneck between the graph and textual views. \emph{(4) About Extensive Experiments:} We conduct comprehensive experimental evaluations for three graph tasks, and experimental results on $11$ real-world public datasets with $20$ compared methods show the superiority of our \methodbase.






==> Chapter/method.tex <==


\begin{figure}[t]
    \centering
    \label{fig:frame}
\includegraphics[width=1\linewidth]{Fig/frame1.0.pdf}
    \caption{The overall framework of \methodbase. In the left part, a parameter-free mechanism is employed to generate the desired output without any additional task-specific training. In the right part, the  Curvature-Aware Graph Representation Learning is designed to align the embeddings between textual and graph views based on the graph curvature.
    }
\end{figure}

\section{Methodology}
%In this section, we mainly introduce the details of the proposed \methodbase framework. Firstly, we formally formulate
%the problem definition and provide an overview  of \methodbase architecture. Then, we introduce the two main components in proposed \methodbase: (1) the training-free textual prompt mechanism aims at exploiting additional textual information from prompts to guide the LLMs to generate refined representations without parameter training and (2) the curvature-aware graph representation learning is to exploit the edge attributes of the curvature to enhance the graph-textual understanding capabilities for downstream tasks. 





\subsection{Problem Statement and Architecture Overview}

The goal of our proposed \methodbase method is to inject the signals of edge attributes into the existing learning paradigm for the graph-driven LLMs to improve the  generalization ability of LLMs for text contents with graph structures, e.g., text-attributed graphs (TAGs). Specifically, given the original node feature $\boldsymbol{X}$ of the graph and textual sequence $\boldsymbol{S} = \{\boldsymbol{S}_1, \boldsymbol{S}_2, \dots, \boldsymbol{S}_i, \dots \boldsymbol{S}_N \}$ for each node, we use the frozen LLM and graph encoder that have been well pre-trained on large-scale datasets to obtain the embeddings $\boldsymbol{X}^{txt} \in \mathbb{R}^{N \times d_t}$ and $\boldsymbol{X}^{gra} \in \mathbb{R}^{N \times d_g}$ under the textual and graph views, respectively. 
%
Here, $N$ is the number of nodes in the graph structure, $d_t$ and $d_g$ are the dimensions of the latent space, and $\boldsymbol{S}_i$ means the textual contents of the model input for the $i$-th node. Enhanced by the adjacency matrix $\boldsymbol{A} \in \mathbb{R}^{N \times N}$ and edge curvature $\boldsymbol{\kappa} \in \mathbb{R}^{N \times N}$, our proposed \methodbase can generate the aligned fusion embedding $\boldsymbol{X}^f \in \mathbb{R}^{N \times d}$, where the values of $\boldsymbol{A}_{ij}$ means the connection relations between nodes $i$ and $j$ and $\boldsymbol{\kappa}_{ij}$ is the value of curvature for $edge(i,j)$. Note that, after extracting the refined final embedding, we fed the fusion embedding $\boldsymbol{X}^f$ to the different heads of various downstream tasks (we focus on three main graph tasks in this paper: node classification, link prediction and graph question answering). 
%
In summary, the inputs of our \methodbase are the node feature $\boldsymbol{X}$, the adjacency matrix $\boldsymbol{A}$ and the textual sequence $\boldsymbol{S}$. The outputs are the refined fusion embedding $\boldsymbol{X}^f$. The overall architecture is provided in Fig. \ref{fig:frame}, which consists of the training-free textual
prompt mechanism and the curvature-aware
graph representation learning.

\subsection{Training-Free Textual
Prompt Mechanism}
Instead of pre-training the LLM for downstream tasks via specific objective engineering \cite{kopf2023openassistant}, we hope to guide the LLM itself to predict the desired output without any
additional task-specific training. Inspired by the success of prompt learning \cite{liu2023pre} with an entirely unsupervised way to solve a great
number of tasks, we propose a novel training-free textual
prompt mechanism to integrate the existing well-pretrained graph-driven LLMs into our \methodbase without training costs. Specifically, our proposed prompt mechanism first exploits two common encoders (textual encoder and graph encoder) to extract the features under textual and graph views, respectively. Then, we initialize and freeze the two encoders using the graph-aware large language model weights which have been well pre-trained on the large corpus of text and graph data. For example, we use the frozen Llama \cite{touvron2023llama} as the textual encoder and a frozen graph encoder in \cite{tape}. 

In order to effectively transfer the textual and graph knowledge from general frozen weights to unknown downstream tasks, our training-free prompt ensemble the techniques for textual-prompt enhancement by constructing diverse task-specific captions, attributes, or high-level concepts of downstream tasks. The more details about designs for the prompt can be referred to {\bf Appendix A.3}. We take the node classification task as an example and 
the general template of the prompt is:
\begin{equation}
\begin{aligned}
&\textit{Here is the abstract of a paper: [\textbf{ABSTRACT}];   
This paper belongs to the [\textbf{TOPIC}];} \\
&\textit{The title of
this paper is [\textbf{TITLE}]; [\textbf{OTHER PROMPTS}];  Now you are a predictor for [\textbf{TASK}];}    \\
&\textit{Please predict this paper may belong to what category and explain the reasons [\textbf{EXPLAINATION}].}
\label{prompt}
\end{aligned}
\end{equation}
The above locations \textit{ [\textbf{ABSTRACT}], [\textbf{TOPIC}], [\textbf{TITLE}]} are the data-specific textual prompts and \textit{ [\textbf{TASK}], [\textbf{EXPLAINATION}]} are the task-specific hand-crafted prompts. The identifier \textit{[\textbf{OTHER PROMPTS}]} means that readers can optionally add relevant prompts meeting the requirements for various tasks to enhance the transferability of LLMs without any additional task-specific training. For node $i$ with the feature $\boldsymbol{X}_i$ and its textual data $\boldsymbol{\hat{S}}_i = \{ \boldsymbol{S}^P_{i,1}, \dots, \boldsymbol{S}^P_{i, L_P}, \boldsymbol{S}_{i, 1}, \dots, \boldsymbol{S}_{i, L_I} \}$, where $L_P$ and $L_I$ are the length of prompts and the original text, we can extract the low-dimensional representation by the frozen LLM and graph encoder. The above process can be formulated as 
\begin{equation}
\begin{aligned}
\boldsymbol{X}_i^{txt} = EncoderLLM(\boldsymbol{\hat{S}}_i), \quad \boldsymbol{X}_i^{gra} = EncoderGraph(\boldsymbol{X}_i).
\label{Frozen_encoder}
\end{aligned}
\end{equation}
Here, $\boldsymbol{S}^P, \boldsymbol{S}$ are the textual tokens of prompts and original inputs respectively, and $\boldsymbol{\hat{S}}$ is the concatenated textual contents. Then, the textual representation  $\boldsymbol{X}^{txt} \in \mathbb{R}^{N \times d_t}$ and graph representation $\boldsymbol{X}^{gra} \in \mathbb{R}^{N \times d_g}$ are fed to the next curvature-aware graph representation learning for fusion, where $N$ is the number of nodes and $d_t, d_g$ are the dimension of latent embeddings. 
%
Compared with existing prompt learning \cite{liu2024can, DBLP:conf/acl/HanCBS24}, the advantages of our proposed training-free textual prompt mechanism are: (1) Since only frozen weights are used for graph and textual encoders, our mechanism can easily ensemble existing graph-aware LLMs that have been pre-trained on other datasets; (2) Due to no need for training from scratch, our mechanism can avoid the additional computational overhead.





\subsection{Curvature-Aware
Graph Representation Learning}

After the enhancement by our training-free textual prompt mechanism, we aim to learn the refined graph-textual fusion representation for improving the performance for various downstream tasks. From the previous discussion in Section \ref{motivation_theorem}, we can learn that the existing fusion mechanism only considers the node information while ignoring the edge attributes may lead to suboptimal solutions (Refer to {\bf Theorem 1}). By discussing curvatures for edge attributes, we can know the edges with negative curvature are the main reason for the information bottleneck between the graph and textual views (Refer to {\bf Theorem 2}). Therefore, we design a curvature-aware graph representation learning to enhance the textual and graph representation fusion. Our representation learning contains two steps: (1) the positive curvature-aware message transport and (2) the enhanced graph aggregation refining. To calculate the curvature for text and graph alignment, we first project textual and graph embeddings into the same curvature space. The above process for projected representations $\boldsymbol{\hat{X}}^{txt} \in \mathbb{R}^{N \times d}$ and $\boldsymbol{\hat{X}}^{gra} \in \mathbb{R}^{N \times d}$ can be written as
\begin{equation}
\begin{aligned}
\boldsymbol{\hat{X}}^{txt} = MLP(\boldsymbol{X}^{txt} | \boldsymbol{\theta}_t), \quad \boldsymbol{\hat{X}}^{gra} = MLP(\boldsymbol{X}^{gra} | \boldsymbol{\theta}_g).
\label{Projector_curvature}
\end{aligned}
\end{equation}
Here, $\boldsymbol{\theta}_t$ and $\boldsymbol{\theta}_g$ are the learnable parameters in the specific multilayer perceptron (MLP).

Because the negative curvature may hinder the information transport, our \methodbase considers aligning the textual and graph representations based on the positive curvatures. Specifically, in our first step of positive curvature-aware message transport, we extend the concept of curvature in Equation \eqref{ricii_curvature} to the scenarios for graph-driven LLMs. Since the probability measure $\boldsymbol{m}$ in curvature is used for neighbor information, we can use the one-hop graph propagation to aggregate the nodes of neighbors, where $\boldsymbol{m}$ can be calculated by $ \boldsymbol{m}_i = \sum_{k \in \mathcal{N}(i)} \boldsymbol{A}_{ik} \boldsymbol{\hat{X}}^{txt}_k$ and $ \boldsymbol{m}_j = \sum_{k \in \mathcal{N}(j)} \boldsymbol{A}_{jk} \boldsymbol{\hat{X}}^{gra}_k$ for node $i$ and $j$ under textual and graph views, respectively. Then, the Equation \eqref{ricii_curvature} can be reformulated:
\begin{equation}
\begin{aligned}
\boldsymbol{\kappa}_{ij} = 1 - \frac{W(\boldsymbol{m}_i, \boldsymbol{m}_j)}{d(\boldsymbol{\hat{X}}^{txt}_i, \boldsymbol{\hat{X}}^{gra}_j)}, 
\label{graph_ricii_curvature}
\end{aligned}
\end{equation}
where $W(\boldsymbol{m}_i, \boldsymbol{m}_j)$ is called the Wasserstein distance (or Earth Mover distance), which is often exploited in the field of optimal transport \cite{DBLP:conf/nips/Wu0ZWL24} or multi-modal alignment \cite{lin2023contrastive}. The above Wasserstein distance can be obtained by solving the following optimal transportation plan:
\begin{equation}
\begin{aligned}
\min_{M} \sum_{i,j} d(\boldsymbol{m}_i, \boldsymbol{m}_j) M(\boldsymbol{m}_i, \boldsymbol{m}_j) \quad \text{s.t.} \sum_j M(\boldsymbol{m}_i, \boldsymbol{m}_j) = 1/N,\ \forall i; \sum_i M(\boldsymbol{m}_i, \boldsymbol{m}_j) = 1/N,\ \forall j.
\label{optimal_transport}
\end{aligned}
\end{equation}
Here, $M(\boldsymbol{x}_i, \boldsymbol{x}_j)$ is the optimal transportation plan from textual node $i$ to graph node $j$ and $d(\boldsymbol{m}_i, \boldsymbol{m}_j)$ is the geodesic distance. In the  {\bf Theorem 2}, we filter the negative curvatures and perform the inter-view message passing only depending on positive curvature ($d(\boldsymbol{\hat{X}}^{txt}_i, \boldsymbol{\hat{X}}^{gra}_j) \textgreater W(\boldsymbol{m}_i, \boldsymbol{m}_j)$). Therefore, we design a novel transport mechanism while filtering the edge with negative curvatures as 
\begin{equation}
\begin{aligned}
\boldsymbol{T}_{ij}= ReLU(d(\boldsymbol{\hat{X}}^{txt}_i, \boldsymbol{\hat{X}}^{gra}_j) - W(\boldsymbol{m}_i, \boldsymbol{m}_j)),
\label{new_transport}
\end{aligned}
\end{equation}
where $\boldsymbol{T} \in \mathbb{R}^{N \times N}$ is the new transportation plan from textual nodes to graph nodes while filtering the negative curvatures and $ReLU(\cdot)$ is the activation function of Rectified Linear Unit (ReLU). Then, we can obtain aligned fusion representations by $\boldsymbol{\hat{X}} = \lambda\boldsymbol{\hat{X}}^{gra} +  (1-\lambda)\boldsymbol{T}\boldsymbol{\hat{X}}^{txt}$.

Although the above fusion mechanism can effectively inject positive curvature information, the direct filtering of $edge(i,j)$ with negative curvature inevitably destroys the edge connection information between nodes $i$ and $j$. To alleviate the problem, we propose the enhanced graph aggregation refining. Specifically, after obtaining the fusion representations $\boldsymbol{\hat{X}} \in \mathbb{R}^{N \times d}$, we perform the graph aggregation for each node to refine the node representations by
\begin{equation}
\begin{aligned}
\boldsymbol{X}^{f} = GNN(
\boldsymbol{\hat{X}}, \boldsymbol{A} | \boldsymbol{\theta}),
\label{FM:GCN}
\end{aligned}
\end{equation}
where $\boldsymbol{\theta}$ is the trainable parameter in the graph neural network (GNN). The explanation of Equation \eqref{FM:GCN} is: For $edge(i,j)$ with negative curvature, the message between $i$ and $j$ can be seen as a two-stage updating, where the node $i$ can first transfer the information to the intermediate node $k$ with positive curvature, and then the infomation may be transferred to node $j$ through graph convolution ($i \xrightarrow{Equation \eqref{new_transport}} k \xrightarrow{Equation \eqref{FM:GCN}} j$). After the graph refining, we can obtain our final textual-graph fusion representation $\boldsymbol{X}^f \in \mathbb{R}^{N \times d}$, which is fed to the different heads for various downstream tasks. Here we take the node classification task as an example, where the head is an $MLP(\cdot)$ function. The above process can be written as
\begin{equation}
\begin{aligned}
\mathcal{L} = CrossEntropy(\boldsymbol{Y}, \boldsymbol{\hat{Y}}) \quad s.t. \quad \boldsymbol{\hat{Y}} = head(\boldsymbol{X}^f) = \sigma(
\boldsymbol{{X}}^{f}\boldsymbol{W} + \boldsymbol{b}).
\label{PLM_Pretrained}
\end{aligned}
\end{equation}
The prediction matrix $\boldsymbol{\hat{Y}} \in \mathbb{R}^{N \times C}$ is the predicted results by our \methodbase, where $C$ is the number of categories. $\boldsymbol{W} \in \mathbb{R}^{d \times C}$ and $\boldsymbol{b}$ are the learnable weight and bias in $head(\cdot)$ function.


% (embedding distance). Then, we can have:

==> Chapter/preliminary.tex <==


%\vspace{-10pt}

\section{Theoretical Motivation and Preliminary}
\label{motivation_theorem}

In this section, we first theoretically analyze the error risk upper bound and the existing message passing function for graph representation learning by LLMs to illustrate our two main motivation: (1) the existing paradigm for graph LLMs using only node alignment while ignoring the structural information of edges can lead to suboptimal solutions and (2) negatively curved edges are
those causing the graph bottleneck and thus leading to the partially indistinguishable phenomenon. Then, some basic concepts and the background of prompt learning are introduced.


\noindent{\bf Theoretical Motivation.} Firstly, we analyze the Generalization Error Upper Bound~\cite{DBLP:conf/icml/CaoXDZH24} of graph representation learning for large language models. The smaller the upper bound of the
generalization error, the better generalization ability for the model. Given the graph $\mathcal{G} = (\mathcal{X}, \mathcal{Y}, \mathcal{E})$, we define the training set $\mathcal{D} = \{(\boldsymbol{x}_i,\boldsymbol{y}_i)\}_{i=1}^N  \in \mathcal{X} \times \mathcal{Y}$, where $\mathcal{X}, \mathcal{Y}, \mathcal{E}$ are the node, label and edge sets. Then, we denote
the graph projection function $f(\boldsymbol{x}): \mathcal{X} \rightarrow \mathcal{Y}$ and $f(\boldsymbol{x})$ is related to the information of the node itself and the aggregation mechanism through the edges. Therefore, the function $f(\boldsymbol{x})$ can be defined as $f(\boldsymbol{x}) = \omega_n f_n(\boldsymbol{x}_n) + \omega_e f_e(\boldsymbol{x}_e)$, where $\omega_n$ and $\omega_e$ are the confidence weights for nodes and edges respectively. When defining $\ell$ as a convex logistic loss function, we can obtain the following theorem and the
full proof of {\bf Theorem 1 } is given in {\bf Appendix A.1}. 

\noindent
{\bf Theorem 1. }(Error Upper Bound for Graph Representation Learning in LLMs) \emph{Let $\hat{e}(f_n)$ and $\hat{e}(f_e)$ denote the empirical errors
of nodes and edges in the graph, respectively. and $\mathcal{H}$ is
hypothesis set, where $f \in H$, and 
$\mathcal{R}_N(\mathcal{H})$ is the Rademacher complexities~\cite{trappenberg2018fundamentals}. With a confidence level of $1-\Delta$
$(0 < \Delta < 1)$
, we have generalization error (GE):
}

\begin{equation}
\begin{aligned}
GE(f) & \leq  2\mathcal{R}_N(\mathcal{H}) + \sqrt{ \frac{2\ln(1/\Delta)}{N} } 
+ \hat{{e}}(f_n) + \hat{{e}}(f_e) \\ 
& + \frac{1}{2} \Bigg[ \underbrace{Cov(\omega_n, \ell_n)}_{\text{Node Covariance}} +
 \underbrace{ Cov(\omega_e, \ell_e)}_{\text{Edge Covariance}} \underbrace{- Cov(\omega_n, \ell_e) - Cov(\omega_e, \ell_n)}_{{\text{Node-Edge Covariance}}}  \Bigg],
\end{aligned}
\end{equation}
where $Cov(\omega, \ell)$ is the covariance between the confidence weight $\omega$ and the loss $\ell$. Because the empirical errors $\hat{{e}}(f_n), \hat{{e}}(f_e)$ and Rademacher complexities $\mathcal{R}_N(\mathcal{H})$ are constant, the lower $GE(f)$ bound is achieved when $Cov(\omega_n, \ell_n) \textless 0$, $Cov(\omega_e, \ell_e) \textless 0$ and $Cov(\omega_n, \ell_e) \textgreater 0$, $Cov(\omega_e, \ell_n) \textgreater 0$ are satisfied.
%
{\bf Theorem 1} shows not only that the generalization ability of the model also depends on the edge structure, but also how the edge information should vary with the nodes. Specifically, node and edge covariances ($Cov(\omega_n, \ell_n) \textless 0$ and $Cov(\omega_e, \ell_e) \textless 0$) imply that when the node or edge embeddings are trained well enough for message passing, we should increase the weights of these nodes and edges. On the contrary, the node-edge covariance ($Cov(\omega_n, \ell_e) \textgreater 0$ and $Cov(\omega_e, \ell_n) \textgreater 0$) suggests that when node information is insufficient for graph propagation, the weights of edges need to be increased to alleviate the above phenomenon.

Secondly, we analyze the existing message passing paradigm for the alignment between the graph and text contents of LLMs and try to explain from a geometric perspective that edges with negative curvature limit the potential for graph representation learning in LLMs.  For the convenience of explanation, we introduce the definitions of the message passing mechanism \cite{wu2023interpretable}.

\noindent
{\bf Definition 1.} (Graph Message Passing Mechanism) \emph{Given the adjacency matrix for the graph $\mathcal{G} = (\mathcal{X}, \mathcal{Y}, \mathcal{E})$ with $d$-dimensional representations, we denote the hidden representation of node $i$ at layer $l$ as $\boldsymbol{h}_i^{(l)}$, where $\boldsymbol{h}_i^{(0)} = \boldsymbol{x}_i$.
Assume that message
function is $\psi_l$ and the update function is $\phi_l$, the graph message passing mechanism can be reformulated as}
\begin{equation}
\begin{aligned}
\boldsymbol{h}_i^{(l+1)} = \phi_l ( \boldsymbol{h}_i^{(l)}, \sum_{j=1}^{n} \boldsymbol{A}_{ij} \psi_l ( \boldsymbol{h}_i^{(l)}, \boldsymbol{h}_j^{(l)} ) ).
\label{graph_message_passing}
\end{aligned}
\end{equation}
Then, we introduce the definition of curvature \cite{li2022curvature} to further analyze the graph mechanism. Following the previous works about the Ollivier-Ricci curvature~\cite{ye2019curvature}, the curvature of the edge between nodes $i$ and $j$ can be written as
% \begin{equation}
% \begin{aligned}
% \min_{M} \sum_{i,j} d(\boldsymbol{x}_i, \boldsymbol{x}_j) M(\boldsymbol{x}_i, \boldsymbol{x}_j) \quad \text{s.t.} \sum_j M(\boldsymbol{x}_i, \boldsymbol{x}_j) = m_x^{\alpha}(i),\ \forall i; \sum_i M(\boldsymbol{x}_i, \boldsymbol{x}_j) = m_x^{\alpha}(j),\ \forall j
% \label{optimal_transport}
% \end{aligned}
% \end{equation}
% where $M(\boldsymbol{x}_i, \boldsymbol{x}_j)$ is the optimal transportation plan from node $i$ to $j$ and $d(\boldsymbol{x}_i, \boldsymbol{x}_j)$ is the geodesic distance
% (embedding distance). Then, we can have:




\noindent
{\bf Definition 2.} (Graph Ollivier-Ricci Curvature) \emph{Given the the graph $\mathcal{G} = (\mathcal{X}, \mathcal{Y}, \mathcal{E})$, we denote the set of neighboring nodes of a node $i \in \mathcal{X}$ as $\mathcal{N}(i)$ and 
a probability measure $\boldsymbol{m}_x^\alpha$ with
a parameter $\alpha$ within $[ 0, 1 ]$. For any edge between node $i$ and $j$, 
the coarse Ricci curvature $\boldsymbol{\kappa}$ on edge
$(i, j)$ is defined by comparing the Wasserstein distance $W(\boldsymbol{m}_i, \boldsymbol{m}_j)$ to the distance d(i, j):}
\begin{equation}
\begin{aligned}
\boldsymbol{\kappa}_{ij} = 1 - \frac{W(\boldsymbol{m}_i, \boldsymbol{m}_j)}{d(i, j)} 
 \quad \text{s.t.} \quad 
  \boldsymbol{m}_x^{\alpha}(i) = 
\begin{cases}
\alpha & \text{if } x = i \\
\frac{1 - \alpha}{k} & \text{if } i \in \mathcal{N}(x) \\
0 & \text{otherwise}
\end{cases}.
\label{ricii_curvature}
\end{aligned}
\end{equation}
After defining the $r$-layer set $S_r(i) = \{ j\in \mathcal{X}: d_G(i,j) = r\}$ and degrees of nodes $i, j$ as $d_i, d_j$, where $d_G$ is the standard shortest-path distance on the graph and $r \in \mathbb{N}$ is the receptive field in graph message passing, we can obtain {\bf Theorem 2} and  the full proof is given in {\bf Appendix A.2}.

{\bf Theorem 2.} (Negative Curvature in Graph Representation Learning with LLMs) \textit{Consider message passing and curvature as in Equation \eqref{graph_message_passing} and \eqref{ricii_curvature}. Let node $i$ under the graph view and node $j$ under the textual view with $d_i \leq d_j$. Assume that the derivatives of functions under graph-graph and text-text message passing are bounded with $|\nabla \phi_l| \leq \alpha$ \textit{and} $|\nabla \psi_l| \leq \beta$, and the message passing functions between graph-text nodes are bounded with $|\nabla \phi_l^{\prime}| \leq \alpha^{\prime}$ \textit{and} $|\nabla \psi_l^{\prime}| \leq \beta^{\prime}$, \textit{for each} $0 \leq l \leq L-1$, \textit{with} the depth of message passing $L \geq 2$. Following \cite{DBLP:conf/iclr/ToppingGC0B22}, \textit{there exists $\delta$ and $\gamma_{\text{max}}^{-1}$ such that } $0 < \delta < \left(\max\{d_i, d_j\}\right)^{-\frac{1}{2}},\ \delta < \gamma_{\text{max}}^{-1}$ \textit{and } $\boldsymbol{\kappa}_{ij} \leq -2 + \delta$.}
\textit{Then given $Q_j \subseteq S_2(i)$ satisfying $|Q_j| > \delta^{-1}$ and for $0 \leq l_0 \leq L - 2$, we have}
\begin{equation}
\begin{aligned}
\frac{1}{|Q_j|} \sum_{k \in Q_j} \left| \frac{\partial \boldsymbol{h}_k^{(l_0 + 2)}}{\partial \boldsymbol{h}_i^{(l_0)}} \right| < (\alpha \beta) ( \alpha^{\prime} \beta^{\prime}) \delta^{\frac{1}{4}}.
\label{negative_ricii_curvature}
\end{aligned}
\end{equation}
The interpretability of {\bf Theorem 2} is that if we
have a negative curvature for $edge(i,j)$ ($\boldsymbol{\kappa}_{ij} \leq -2 + \delta$), there may exist a large number of nodes $k$ ($k \in Q_j$), where the message passing from node $i$ under the graph view to nodes $k$ under textual view is affected, despite the distance is $2$ for these nodes $k$ to node $i$ (from layers $l_0$ to $l_0 + 2$).

\noindent{\bf Preliminary for Prompt Learning.} Prompt learning \cite{DBLP:conf/nips/Castillo-Bolado24} is an effective fine-tuning strategy to advance the generalization from LLMs to a specific downstream task \cite{sun2024prompt}. Specifically, these prompt-based approaches \cite{DBLP:conf/nips/0001L00024, DBLP:conf/nips/0001MZ0GP24} usually add a small
number of additional embeddings (e.g., the explanation why the model makes the prediction or a detailed description for the task) along with model inputs, while  the LLM
models are kept frozen. In this paper, our prompts are textual forms including additional information or constraints to guide behaviors of the model, such as a single sentence for the title of a node or a longer passage for the description of a specific task. Formally, the training process of LLMs can be defined to optimize a conditional probability distribution $p(\boldsymbol{y}|\boldsymbol{s})$, where $\boldsymbol{s} = (\boldsymbol{s}_1, \dots, \boldsymbol{s}_{L_I})$ is  a textual sequence of tokens for model inputs and $L_I$ is the length of the input sentences. After introducing the prompt $\boldsymbol{s}^p = (\boldsymbol{s}^p_1, \dots, \boldsymbol{s}^p_{L_P})$, the new paradigm of LLMs can be reformulated to compute the conditional probability distribution $p(\boldsymbol{y}|\boldsymbol{\hat{s}}) = \prod_{i=1}^{m} p(\boldsymbol{y}_i \mid \boldsymbol{y}_{<i}, \boldsymbol{\hat{s}})$. Here $\boldsymbol{\hat{s}} = (\boldsymbol{s}^p_1, \dots, \boldsymbol{s}^p_{L_P}, \boldsymbol{s}_1, \dots, \boldsymbol{s}_{L_I})$ is the token sequence obtained by concatenating the textual prompt $\boldsymbol{s}^p$ and input $\boldsymbol{s}$. The probability $p(\boldsymbol{y}|\boldsymbol{\hat{s}}) = \prod_{i=1}^{m} p(\boldsymbol{y}_i \mid \boldsymbol{y}_{<i}, \boldsymbol{\hat{s}})$ means the
probability of generating token $\boldsymbol{y}_i$ given $\boldsymbol{y}_{<i}$ and $\boldsymbol{\hat{s}}$. More details about the {\bf Related Work} can be found in {\bf Appendix A.3.}



%\noindent{\bf Preliminary for PLM.} A Pretrained Language Model (PLM) framework consists of a multi-layer transformer
%encoder that takes a sentence $\mathbb{S}$ as input and outputs the hidden
%states $\boldsymbol{h}$ of each token. The formulation of the above process can be formulated as 
%$\{\boldsymbol{h}_0,\dots, \boldsymbol{h}_{L_s} \} = Transformer(\{\boldsymbol{s}_0,\dots, \boldsymbol{s}_{L_s} \})$, where $\boldsymbol{s}$ is the token in the sentence $\mathbb{S} = \{\boldsymbol{s}_0,\dots, \boldsymbol{s}_{L_s} \}$ and $L_s$ is the length of the sentence. To pretrain the above PLM framework, an auto-regressive mechanism \cite{DBLP:conf/www/HuangHYBTCZ24} is exploited to minimize the negative log-likelihood. Specifically, the language model needs to predict the probability distribution of the next token $k$ based on the previous tokens $\{0,\dots,k-1 \}$ and the formulation can be written as 
%\begin{equation}
%\begin{aligned}
%\mathcal{L}_p = \sum_{k=1}^{L_s}CrossEntropy(\boldsymbol{\hat{s}}_k, \boldsymbol{s}_k) \quad s.t. \quad \boldsymbol{\hat{s}}_k = p(\boldsymbol{s}_i|\boldsymbol{s}_0,\dots, \boldsymbol{s}_{k-1}) = head(\boldsymbol{h}_k),
%\label{PLM_Pretrained}
%\end{aligned}
%\end{equation}
%where $\boldsymbol{\hat{s}}_k$ and $ \boldsymbol{s}_k$ are the predicted value and ground truth, respectively. The function $head(\cdot)$ in the loss function $\mathcal{L}_p$ means the language model head to generate the textual contents and  $p(\cdot)$ is the joint probability of the sequence.
